Ricci Flow Emerging from Rotationally Symmetric Degenerate Neckpinches

In previous work, Angenent, Isenberg, and Knopf created type-II Ricci flow neckpinch singularities. In this paper we construct solutions to Ricci flow whose initial data is the singular metric resulting from these singularities. We show in particular that the curvature decreases at the same rate at which it blew up. This is the first example of Ricci flow starting from a type-II singularity.

==> constant_digraph.tex <==

\begin{tikzpicture}
  [scale=.8,auto]
  \node (r) at (0,8) {$r_*$};
  \node (e) at (9,8)  {$\epsilon$};
  \node (d) at (13,8)  {$\delta$};
  \node (p) at (3,6) {$\rho_*$};
  \node (D) at (7,4)  {$D$};
  \node (g) at (13,4)  {$\gamma_\pm$};
  \node (s) at (3,2)  {$\sigma_*$};
  \node (k) at (13,0)  {$\kappa_\pm$};

  \draw [->] (r) to node {B1} (p);
  \draw [->] (e) to node {G1} (p);
  \draw [->] (e) to node {G1} (g);
  \draw [->] (d) to node {G1} (g);
  \draw [->] (p) to node {B2} (D);
  \draw [->] (p) to node {B2, G2} (s);
  \draw [->] (g) to node {G2} (k);
  \draw [->] (D) to node {G2} (k);
  \draw [->] (D) to node {B2, G2} (s);
  \draw [->] (s) to node {G2} (k);

  % \draw [->] (r) to node {\ref{ourouterbarriertheorem}} (p);
  % \draw [->] (e) to node {\ref{paraoutglue}} (p);
  % \draw [->] (e) to node {\ref{paraoutglue}} (g);
  % \draw [->] (d) to node {\ref{paraoutglue}} (g);
  % \draw [->] (p) to node {\ref{parabarriertheorem}} (D);
  % \draw [->] (p) to node {\ref{parabarriertheorem}, \ref{inoutglue}} (s);
  % \draw [->] (g) to node {\ref{inoutglue}} (k);
  % \draw [->] (D) to node {\ref{inoutglue}} (k);
  % \draw [->] (D) to node {\ref{parabarriertheorem}, \ref{inoutglue}} (s);
  % \draw [->] (s) to node {\ref{inoutglue}} (k);
  
\end{tikzpicture}


==> soln_beforecrazy.tex <==
\section{Bounds yielding convergence to a regularized solution}
\label{sec:conv}

\subsection{Basic Curvature Bound}
This lemma lets us understand the curvature of the sub- and supersolutions created above.

\begin{lemma}\label{curvaturebnd}
  Let $v(r, t)$ is a solution to $v_t = \fop[v]$ on $(0, r_*) \times (0, t_*)$.  Suppose that $v$ satisfies $v^- < v < v^+$, as well as the assumptions \ref{vbnd} and \ref{abnd} on the initial data, i.e. that
  $$|v(r, t)| < 1, \qquad \text{for }r>0,$$
  $$|r^2 (L-K)| = |(1-v)+\frac{1}{2}rv_r| < A.$$
  Then for some $C$
  $$
  \left| \frac{1-v}{r^2} \right| + \left| \frac{v_r}{2r} \right| 
  \leq C\frac{1}{t^{b+1}}
  $$
\end{lemma}

\begin{proof}
  The fact that $v$ lies between our subsolution and supersolution will give us an immediate bound on $|L|$.  As we mentioned when describing the initial data, we will have to use the bound on $|r^2 (L-K)|$ to bound $K$.

  As $v < 1$,
  $$\left| \frac{1-v}{r^2} \right| = \frac{1-v}{r^2} \leq \frac{1-v^-}{r^2}$$
  Outside of the inner region, by definition $\sigma \geq \sigma_*$, which translates to
  $\frac{1}{r^2} \leq \frac{1}{\sigma_*^2 t^{b+1}}.$
  In particular $|L| \leq C\frac{1}{t^{b+1}}$.
  In the inner region, we have 
  $$\left| \frac{1-v}{r^2} \right| \leq \frac{1-v_{\inner}^-}{r^2} = \frac{1-\bry (k_-\sigma) + (1-\epsilon) k^{-2}_- \cry(k_-\sigma)\theta \theta_t}{r^2}.$$
  which, checking the asymptotics of $\bry$ and $\cry$, gives the bound
  $$|L| = \left| \frac{1-v}{r^2} \right| \leq C \frac{\sigma^2 }{r^2} = C \frac{1}{t^{b+1}}.$$
  Thus, the bound $|L| \leq C\frac{1}{t^{b+1}}$ holds throughout.

  Now we apply the bound on $|L-K|$ from the hypotheses:
  $$|K| \leq |L| + \frac{A}{r^2} \leq C \left( \frac{1}{t^{b+1}} + \frac{1}{r^2} \right)$$

  Outside of the inner region, $\frac{1}{r^2}$ is dominated by $\frac{1}{t^{b+1}}$.  Therefore the bound $|K| \leq C \frac{1}{t^{b+1}}$ follows for $\frac{r^2}{t^{b+1}}<\sigma_*^2$.
  
  In the inner region, the rescaling argument from \cite[lemma~10]{ACK} carries through.  For arbitrary $(\bar r, \bar t)$ in the inner region, consider
  $$w(x, y)
  = \bar \sigma^{-2} (1 - v(\bar r + \bar r x, \bar r + \bar r^2 y))
  = \frac{\bar t^{b+1}}{\bar r^2}(1 - v(\bar r + \bar r x, \bar r + \bar r^2 y)).
  $$
  One checks that $w$ is bounded and solves a strictly parabolic equation on $[-\frac{1}{2}, \frac{1}{2}] \times [-\frac{1}{2}, \frac{1}{2}]$.  (The coefficient of $w_{xx}$ is $1-\bar \sigma^2w = v$, which is bounded from below in the inner region.)  Furthermore, $w$ and the ellipticity constant are bounded independently of $(\bar r, \bar t)$.  Applying interior estimates yields $w_x(0,0) < C$ for some constant independent of $(\bar r, \bar t)$, and scaling back we find $v_r(\bar r, \bar t) < C\frac{1}{\bar t^{b+1}}$.
  
  
\end{proof}
\subsection{Maximum Principles}
In \cite{ACK}, the authors state and prove the following maximum principle.
\begin{lemma}\label{maxprinc}
  Let $v^-$ and $v^+$ be nonnegative, piecewise smooth, sub- and supersolutions of $v_t = \fop[v]$, that is:
  $$\left( \pars{}{t} - \fop \right) v^+ \geq 0 \qquad \left( \pars{}{t} - \fop \right) v^- \leq 0$$
  Assume either $v^-$ or $v^+$ satisfies
  $$v_{rr} \leq C, \qquad -\frac{v_r}{2r} \leq C, \qquad \frac{1-v}{r^2} \leq C$$
  for some $C<\infty$, on $\Xi = [0, \bar r] \times [0, \bar t]$.

  If $v^-(\bar r, t) \leq v^+(\bar r, t)$ and $v^-(0, t) \leq v^+(0, t)$ hold for $0 \leq t \leq \bar t$, and $v^-(r, 0) \leq v^+(r, 0)$ holds for $0 \leq r \leq \bar r$,  then $v^- \leq v^+$ holds throughout $\Xi$.
\end{lemma}

We need a way to verify the inequality on the right edge of the domain $r = \bar r$ in the hypothesis of the theorem above.  To do this, we will use the following barriers from \cite{ACK}.

\begin{lemma}\label{collarthm}
  For any $0 < m < 1$, $\bar r >0$, and small enough $\alpha > 0$, there exists $T = T(\alpha) >0$ such that for $0 < t < T(\alpha)$, the functions
  $$v_{\text{col}}^-(r, t) =
  \max
  \left\{
  0, m_-e^{-t/\alpha^2} - \left( \frac{r-\bar r}{\alpha} \right) ^2
  \right\}
  $$
  $$v_{\text{col}}^+(r, t) =
  \min
  \left\{
  1, m_+e^{3t/\alpha^2} + \left( \frac{r-\bar r}{\alpha} \right) ^2
  \right\}
  $$
  are sub- and supersolutions of $v_t = \fop[v]$, respectively.
\end{lemma}

The following maximum principle is the analogue to Lemma 2 of $\cite{ACK}$.  It allows us to conclude that there are no noncompact solutions coming out of the singularity, as in Theorem 2 of $\cite{ACK}$.  It also gives an easy diameter bound.
\begin{lemma}\label{cptnesssubsoln}
  Let $v$ be a nonnegative smooth function satisfying 
  $$v_t \geq \fop[v]$$
  on $(0, r_0] \times [0, t_0]$ and
  $$v(r, 0) \geq r^{2b_*}$$
  where $b_* \in (1/2, 1)$.    Then $v \geq r^{2b_*}$ on $(0, r_1) \times [0, t_1]$ for some small $r_1, t_1$.
\end{lemma}
Notice the hypotheses do not impose boundary conditions at $r=0$, only that the equation is satisfied in the interior.
\begin{proof}
  Let $\bar v(r) = r^{2b_*}$.  Choose $r_1 = \left( \frac{ab}{2b^2+b+a} \right) ^{1/4b}$, or $r_1 = r_0$ if that is smaller.  Demand that $t_1$ is small enough so that $\bar v(r_1) < v(r_1, t)$ for $0 \leq t \leq t_1$.
  For arbitrary $\epsilon > 0$ let
  $$f_\epsilon(r, t) = v(r, t) - \bar v (r)  + \epsilon (1+t).$$
  We prove $f_\epsilon(r, t) > 0$ for $0 < r < r_1$.  The lemma follows by sending $\epsilon $ to 0.

  From our demand on $t_0$ and our hypotheses, we have
  $$f_\epsilon(r, 0) \geq \epsilon, \qquad \text{ for all } r \in [0, r_0]$$
  and 
  $$f_\epsilon(0, t) \geq \epsilon, \qquad f_\epsilon(r_0, t) \geq \epsilon,  \qquad \text{ for all } t \in [0, t_0].$$
  Suppose for contradiction we have a first time $\bar t \in (0, t_0]$ where $f_\epsilon$ has a zero, and take $\bar r$ minimal such that $f(\bar r, \bar t) = 0$.

  Then, on one hand, since we have $v_t \geq \fop[v]$,
  \begin{equation}\label{cptnessineq:fopneg}
    0 \geq f_{\epsilon, t}(\bar r, \bar t) \geq \fop[v(\bar r, \bar t)] + \epsilon
  \end{equation}

  On the other hand, we have
  $$0 = f_{\epsilon, r}(\bar r, \bar t), \qquad 0 \leq f_{\epsilon, rr}(\bar r, \bar t)$$
  so at the point $(\bar r, \bar t)$
  $$v < \bar v , \qquad v_r = \bar v_r, \qquad v_{rr} \geq \bar v_{rr}$$
  so
  \begin{align*}
    \bar r^2 \fop[v(\bar r, \bar t) ]
    &=
    \frac{a}{2}\bar rv_r + av
    + \bar r^2 v_{rr}v - \frac{1}{2}(\bar r v_r)^2
    - \bar r v_r v - av^2 \\
    &\geq
    \frac{a}{2}\bar r \bar v_r 
    - \frac{1}{2}(\bar r \bar v_r)^2
    - \bar r \bar v_r \bar v - a\bar v^2 \\
    &=
    abr^{2b}
    - (2b^2 + b + a)r^{4b}
  \end{align*}
  In the first inequality we used that $v$ and $v_{rr}v \geq \bar v_{rr} v$ are positive.  From the last line, we see from our choice of $r_1$ above that $\bar r \fop[v(\bar r, \bar t)] > 0$, contradicting (\ref{cptnessineq:fopneg}).
\end{proof}
  
  

\subsection{Regularizations}

We construct the smooth evolution from our singular initial data as the limit of a sequence of regularized metrics.  We will describe the construction of the regularized metrics here.

Let $\Nb_{r_0}$ be the connected neighboorhood of the north pole where $\psi_{init}(x)<r_0$.  Recall $r_\#$ is defined so that $\psi_s > 0$ if $0 < \psi < 2r_\#$.  For small $\omega \geq 0$, we will construct a smooth rotationally-invariant metric $g_\omega = (ds)^2 + \psi_\omega(s)^2 g_{S^n}$ on $S^{n+1}$.   On $S^{n+1}-\Nb_{\rho_* \sqrt{\omega}}$ we let $g_\omega$ coincide with our initial metric $g_{\init}$.  On $\Nb_{\rho_* \sqrt{\omega}}$ we will still have $\psi_s>0$, so we may use $r$ as a coordinate.  There, $v_\omega = \psi_{\omega,s}^2$ satisfies
$$v^-(r, \omega) < v_\omega(r) < v^+(r, \omega)$$
as well as $|r^2(K-L)| < A$.  (Recall this last condition also holds for our initial data $v_{\init}$, and it is preserved under Ricci flow.)

\begin{lemma}[Uniform short time existence]
\end{lemma}

\begin{theorem}\label{regularizedproperties}
  The regularized metrics have a Ricci flow on some time interval $[0, t_*]$, with the following properties.  For small positive $\epsilon, \delta$, let $r_*$ be the corresponding radius for the barriers.
  \begin{itemize}
  \item Outside of $\Nb_{r_*}$, all derivatives of $|\Rm|$ are bounded independently of $\omega$.
  \item In $\Nb_{r_*}$, The slope function $v$ is kept between the sub- and supersolutions,
    $$
    v_{\epsilon, \delta}^-(r, t+\omega)
    < v_\omega(r, t)
    < v_{\epsilon, \delta}^+(r, t+\omega)
    $$
  \item The curvature $|\Rm|$ is bounded by
    $$|\Rm| \leq \frac{C}{t^{b+1}}$$
    where $C$ is independent of $\omega$.  In particular, for fixed $t_1$ the curvature is bounded indepently of $\omega$ or $r$.
  \item For fixed $r_1>0$, the norm of the curvature tensor and all its derivatives are bounded on $S^{n+1} - \Nb_{r_1} \times [0, t_*]$:
    $$|\nabla \Rm| < C_k(r_1), \qquad k = 0, 1, 2, \dots$$
  \item The diameter of the solutions are bounded from above, and the injectivity radius at $\NP$ is bounded from below, independently of $\omega$.  
  \end{itemize}
\end{theorem}

\begin{proof}
  The lower bound $t_*$ on the time that the Ricci flow of $g_\omega$ exists comes from the bound on $r^2(K-L)$, and the fact that $\psi_s>0$ in  $\Nb_{r_\#}$ \cite[p.~8]{ACK}.  Since $\psi_s \leq 1$ and $|r^2(K-L)| = |\psi \psi_{ss}-\psi_s^2 + 1| < A$ we have
  $$|(\psi^2)_t| = |2(\psi \psi_{ss}-\psi_s^2+1) + 2n(\psi_s^2 -1)|  \leq 2(A + n)$$


  Intuitively outside of $\Nb_{r_*}$ there should be no problems with $|\Rm|$ and its derivatives.  See \cite[Lemma~9]{ACK} for details.


    
  Now, we prove that $v_{\omega}$ stays between the sub- and supersolutions.  Figure \ref{figure:collar} illustrates this argument.  Choose the constants $m_{\pm}$ and $\alpha$ in \ref{collarthm} so that
  \begin{equation}\label{initcollartrap}
    v^-_{\col}(r, 0) < v_{\init}(r, 0) < v^+_{\col}(r, 0)
  \end{equation}
  for all $r \in (0, r_\#]$, and 
  \begin{equation}\label{rightedgepinch}
  v^-_{\epsilon, \delta} (r_*, 0) < v^-_{\col}(r_*, 0),
  \qquad
  v^+_{\col}(r_*, 0) < v^+_{\epsilon, \delta}(r_*, 0).
  \end{equation}
  Then shrink $t_0$ so the second inequality (\ref{rightedgepinch}) holds for $0 < t < t_0$.  The first inequality (\ref{initcollartrap}) actually holds for $v_{\init}$ replaced with $v_{\omega}$ (for $\omega$ small enough) since we do not modify $v_{\init}$ near $r_*$, and near 0
  $$v^-_{\col}(r, 0) = 0 < v_{\omega}(r, 0) < 1 = v^+_{\col}(r,0).$$
  Now we apply the maximum principle (Lemma \ref{maxprinc}) twice.  First, we apply it with the collar sub- and supersolutions. For all $\omega$ we have $|\psi_s| < 1$, and this is preserved under Ricci flow.  Since $0 < v(r, t) < 1$ the condition on the right edge of the domain is satisfied.  Therefore $v_\omega$ stays between the collars, in particular
  $$
  v^-_{\epsilon, \delta} (r_*, 0) < v^-_{\col}(r_*, t)
  < v_{\omega}(r_*, t)
  < v^+_{\col}(r_*, t) < v^+_{\epsilon, \delta}(r_*, 0)
  $$
  which allows us to apply the maximum principle to $v^\pm_{\epsilon, \delta}$, on $[0, r_*] \times [0, t_0]$.
  \begin{figure}[t]
    \includegraphics[scale=1]{images/collars.pdf}
    \includegraphics[scale=1]{images/collar_mvmnt.pdf}
    \caption{Left: The collars, separating $v^\pm(r_*, 0)$ from $v_{\init}(r_*)$.  Right: the initial situation (solid) and the situation after a small time (dashed). (The Ricci flow here is completely made up.)
      The collars are still keeping the solution away from $v^\pm(r_*, t)$.}
    \label{figure:collar}
  \end{figure}

  Now that we have $v_{\omega}$ trapped between our sub- and supersolutions, we can apply the curvature bound from lemma \ref{curvaturebnd} to show $|K| + |L| \leq \frac{C}{(t+\omega)^{b+1}} \leq \frac{C}{t^{b+1}}$ , at least in $\Nb_{r_*}$.  Outside of $\Nb_{r_*}$ there are no problems, because of the bounds on $|\Rm|$ there.

  We now show that for fixed $r_1$ the curvature at $r = r_1$ is uniformly bounded, following lemma 11 of \cite{ACK}.  Consider $v_{\omega}(r, t)$ on $[\frac{r_1}{2}, 2r_1] \times [0, t_*]$.  Each $v_{\omega}$ satisfies $v_{\omega, t} = \fop [v_{\omega}]$.  Since $v_{\omega}$ is trapped between our barriers, $\fop$ is elliptic with ellipticity constant strictly away from 0, and the boundary data is uniformly bounded.  So: derivatives of $v_{\omega}$ at $r_1$ are bounded independently of $\omega$ or $t$.  Since $|\Rm|$ can be written in terms of $v$, $\pars{v}{r}$, and $r$,  $|\Rm|$ is bounded at $r = r_1$.

  Because of the bounds on $|\Rm|$ outside of $\Nb_{r_*}$ the diameter cannot change much there.  This also gives a lower bound on the injectivity radius at $\NP$ because geodesics emanating from $\NP$ can only meet at $\SP$.  The upper bound on the diameter inside of $\Nb_{r_*}$ can come from the fact that $v_{\omega}$ is trapped between $v^-_{\epsilon, \delta}$ and $v^+_{\epsilon, \delta}$, or even from Lemma \ref{cptnesssubsoln}.
\end{proof}

\subsection{Convergence to a Solution}

We use the bounds found in the previous subsections to obtain subsequential convergence of the $g_{\omega}$ to a solution of Ricci Flow on $(0, t_*)$, which agrees with our initial metric $g_{\init}$ in the limit as $t \searrow 0$.  Our main tool is Hamilton's compactness result \cite{H}, which we admit may be like cracking a rotationally symmetric nut with a sledgehammer.  Perhaps using a nutcracker made for rotationally symmetric nuts would yield independence of subsequence.

The method in Lemma 12 and Lemma 13 of \cite{ACK} applies perfectly well in our situation.  There, convergences is found on $(S^{n+1}-\Nb_{r_1}) \times [0, t_*]$, and a diagonalization argument takes $r_1$ to $0$, and the convergence to $(S^{n+1}-\NP) \times [0, t_*]$.  Some work must be done to extend the convergence to the north pole $\NP$ at positive times.

We find it simpler, however, to find the convergence on $S^{n+1} \times [t_1, t_*]$, and use a diagonalization argument to take $t_1$ to $0$.  That way, the convergence is done in the nicest possible situation: a compact manifold on a compact time interval.

\begin{theorem}
A subsequence $g_{\omega_j}$ of the regularized solutions converge to a solution $g_{*}$ of Ricci flow on $(0, t_*] \times S^{n+1}$, for some $t_*$.  On $S^{n+1}\setminus \{\NP\}$, $g_{*}$ converges in $C^\infty_{\text{loc}}$ to the initial metric $g_{\init}$.
\end{theorem}
\begin{proof}
  We take $t_*$ small enough to satisfy the finitely many time conditions throughout our arguments.  It's enough to show that such a subsequence of regularized metrics exists on any interval $[t_1, t_*]$; since our convergence doesn't claim to be uniform in time a diagonal argument completes the result.  

  We apply Hamilton's compactness result \cite{H}.  Theorem \ref{regularizedproperties} contains all of the properties we need to apply the result.  In particular
  \begin{itemize}
  \item The norm of the curvature tensor $|\Rm|$ is bounded by $\frac{C}{t_{1}^{1+b}}$, where $C$ is independent of $\omega$.
  \item The injectivity radius at $\NP$ is bounded from below, independently of $\omega$.
  \end{itemize}
  So we get pointed convergence (centered at $\NP$) to some Ricci flow.  Furthermore, because of the diameter bound, the limit must be $S^{n+1}$.  The limit must also be $SO(n+1)$ invariant, with the same poles.

  Now let $v_*(r, t)$ be the slope function corresponding to the 
\end{proof}
